Hyperbolic Disentangled Representation for Fine-Grained Aspect Extraction

Automatic identification of salient aspects from user reviews is especially useful for opinion analysis. There has been significant progress in utilizing weakly supervised approaches, which require only a small set of seed words for training aspect classifiers. However, there is always room for improvement. First, no weakly supervised approaches fully utilize latent hierarchies between words. Second, each seed words representation should have different latent semantics and be distinct when it represents a different aspect. In this paper, we propose HDAE, a hyperbolic disentangled aspect extractor in which a hyperbolic aspect classifier captures words latent hierarchies, and aspect-disentangled representation models the distinct latent semantics of each seed word. Compared to previous baselines, HDAE achieves average F1 performance gains of 18.2% and 24.1% on Amazon product review and restaurant review datasets, respectively. In addition, the em-bedding visualization experience demonstrates that HDAE is a more effective approach to leveraging seed words. An ablation study and a case study further attest to the effectiveness of the proposed components

==> aspect_regularize_dis.tex <==
\begin{table}[t]
\small
\centering
\caption{$\mathit{AUC}$ of \system with different number of $l_\mathrm{p}$,
$l_\mathrm{w}$, and $l_\mathrm{d}$ hops, where $K_m$ is set to 16. For the
Propagation layer, 0 hops denotes that only the user-clicked items $h^{1}_{i}$ are
utilized.} 
\begin{tabular}{p{2.5cm}|cccccc}
\hline \multicolumn{1}{c|}{\multirow{1}{*}{$d_1$ ($\mathcal{P})$/(E) }} & \multicolumn{1}{c}{{4}} & \multicolumn{1}{c}{{8}} & \multicolumn{1}{c}{{16}} &
\multicolumn{1}{c}{{32}} &
\multicolumn{1}{c}{{64}} \\ \hline \multicolumn{1}{c|}{Bags} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{{}} \\ 
\multicolumn{1}{c|}{B/T}  &
\multicolumn{1}{c}{{}} & 
\multicolumn{1}{c}{}   & \multicolumn{1}{c}{{}} & \multicolumn{1}{c}{}   & \multicolumn{1}{c}{{}} \\
\multicolumn{1}{c|}{Boots} &
\multicolumn{1}{c}{}  & 
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{{}} \\
\hline
\end{tabular}
\label{tb:HDAE_by_P_W_D_hops}
%\vspace{-0.5 pc}
\end{table}



% \begin{table}[t]
% \small
% \centering
% \caption{$AUC$ of \system with different number of W and D hops and We set the size of P set to 16.}
% \begin{tabular}{p{2.5cm}|ccc}
% \hline 
% \multicolumn{1}{c|}{\multirow{1}{*}{W hop}} & \multicolumn{1}{c}{{1}} & \multicolumn{1}{c}{{2}} &
% \multicolumn{1}{c}{{3}} \\ \hline \multicolumn{1}{c|}{ML-1M} & 
% \multicolumn{1}{c}{{.9261}} & \multicolumn{1}{c}{{\textbf{.9267}}} &
% \multicolumn{1}{c}{{.9262}}  \\ 
% \multicolumn{1}{c|}{LFM-1b}  & 
% \multicolumn{1}{c}{{.9438}} & \multicolumn{1}{c}{{.9445}} &
% \multicolumn{1}{c}{{\textbf{.9447}}}  \\
% \multicolumn{1}{c|}{AZ-book}  & 
% \multicolumn{1}{c}{{.8568}} & \multicolumn{1}{c}{{.8611}} &
% \multicolumn{1}{c}{{\textbf{.8618}}}  \\
% \hline
% \multicolumn{1}{c|}{\multirow{1}{*}{D hop}} &  \multicolumn{1}{c}{{1}} & \multicolumn{1}{c}{{2}} &
% \multicolumn{1}{c}{{3}} \\ \hline \multicolumn{1}{c|}{ML-1M} & 
% \multicolumn{1}{c}{{.9261}} & \multicolumn{1}{c}{{\textbf{.9269}}} &
% \multicolumn{1}{c}{{.9250}}  \\ 
% \multicolumn{1}{c|}{LFM-1b}  & 
% \multicolumn{1}{c}{{.9438}} & \multicolumn{1}{c}{{\textbf{.9441}}} &
% \multicolumn{1}{c}{{.9440}}  \\
% \multicolumn{1}{c|}{AZ-book}  & 
% \multicolumn{1}{c}{{.8552}} & \multicolumn{1}{c}{{\textbf{.8621}}} &
% \multicolumn{1}{c}{{.8613}} \\
% \hline
% \end{tabular}
% \label{tb:KGPH_by_wide_deep_hops}
% \end{table}



% \begin{table}[t]
% \small
% \centering
% \caption{$AUC$ of \system with different number of D hops.}
% \scalebox{1.0}{
% \begin{tabular}{p{2.5cm}|ccc}
% \hline \multicolumn{1}{c|}{\multirow{1}{*}{D hop}} &  \multicolumn{1}{c}{{1}} & \multicolumn{1}{c}{{2}} &
% \multicolumn{1}{c}{{3}} \\ \hline \multicolumn{1}{c|}{ML-1M} & 
% \multicolumn{1}{c}{{\textbf{.9269}}} & \multicolumn{1}{c}{{.9261}} &
% \multicolumn{1}{c}{{.9250}}  \\ 
% \multicolumn{1}{c|}{LFM-1b}  & 
% \multicolumn{1}{c}{{.9438}} & \multicolumn{1}{c}{{\textbf{.9441}}} &
% \multicolumn{1}{c}{{.9440}}  \\
% \multicolumn{1}{c|}{AZ-book}  & 
% \multicolumn{1}{c}{{.8552}} & \multicolumn{1}{c}{{\textbf{.8621}}} &
% \multicolumn{1}{c}{{.8613}}  \\
% \hline
% \end{tabular}}
% \label{tb:KGPH_by_deep_hops}
% \end{table}



% \begin{table}[t]
% \small
% \centering
% \caption{$AUC$ of \system with different number of W hops.}
% \scalebox{1.0}{
% \begin{tabular}{p{2.5cm}|ccc}
% \hline \multicolumn{1}{c|}{\multirow{1}{*}{D hop}} &  \multicolumn{1}{c}{{1}} & \multicolumn{1}{c}{{2}} &
% \multicolumn{1}{c}{{3}} \\ \hline \multicolumn{1}{c|}{ML-1M} & 
% \multicolumn{1}{c}{{\textbf{.}}} & \multicolumn{1}{c}{{.}} &
% \multicolumn{1}{c}{{.}}  \\ 
% \multicolumn{1}{c|}{LFM-1b}  & 
% \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{\textbf{.}}} &
% \multicolumn{1}{c}{{.}}  \\
% \multicolumn{1}{c|}{AZ-book}  & 
% \multicolumn{1}{c}{{.}} & \multicolumn{1}{c}{{.}} &
% \multicolumn{1}{c}{{\textbf{.}}}  \\
% \hline
% \end{tabular}}
% \label{tb:KGPH_by_wide_hops}
% \end{table}


==> by_trainning_set_2.tex <==
\begin{table}[t]
\small
\centering
\caption{Micro-averaged F1 for 12-class sentence-level aspect detection in restaurant reviews in English with different ratios of training set r.}
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{1}{*}{}} 
& \multicolumn{5}{c|}{Restaurant review domain (En)}
\\
\multicolumn{1}{|l|}{\multirow{1}{*}{ratio r}} &
\multicolumn{1}{c}{10\%}&
\multicolumn{1}{c}{30\%}&
\multicolumn{1}{c}{50\%}&
\multicolumn{1}{c}{70\%}&
\multicolumn{1}{c|}{100\%}\\
\hline \multicolumn{1}{|l|}{{W2V-Gold}} & \multicolumn{1}{c}{{20.5}} &
\multicolumn{1}{c}{{41.6}} &
\multicolumn{1}{c}{{48.7}} &
\multicolumn{1}{c}{{58.9}} &
\multicolumn{1}{c|}{{74.2}}  \\
\multicolumn{1}{|l|}{{BERT-Gold}} & \multicolumn{1}{c}{{28.2}} &
\multicolumn{1}{c}{{41.5}} &
\multicolumn{1}{c}{{55.1}} &
\multicolumn{1}{c}{{63.5}} &
\multicolumn{1}{c|}{{71.7}}  \\
\hline 
\multicolumn{1}{|l|}{{MATE}} &
\multicolumn{1}{c}{{44.3}} &
\multicolumn{1}{c}{{55.3}} &
\multicolumn{1}{c}{{61.2}} &
\multicolumn{1}{c}{{68.8}} &
\multicolumn{1}{c|}{{75.6}}  \\
\multicolumn{1}{|l|}{{TS-ATT}} & \multicolumn{1}{c}{{47.2}} &
\multicolumn{1}{c}{{62.8}} &
\multicolumn{1}{c}{{66.1}} &
\multicolumn{1}{c}{{71.7}} &
\multicolumn{1}{c|}{{75.9}}   \\
\multicolumn{1}{|l|}{{TS-BT}} & \multicolumn{1}{c}{{55.8}} &
\multicolumn{1}{c}{{61.7}} &
\multicolumn{1}{c}{{62.3}} &
\multicolumn{1}{c}{{70.2}} &
\multicolumn{1}{c|}{{73.7}}  \\
\multicolumn{1}{|l|}{{\system}} &
\multicolumn{1}{c}{{\textbf{59.1}}} &
\multicolumn{1}{c}{{\textbf{66.2}}} &
\multicolumn{1}{c}{{\textbf{71.2}}} &
\multicolumn{1}{c}{{\textbf{74.6}}} &
\multicolumn{1}{c|}{{\textbf{79.7}}} \\
\hline 
\end{tabular}
\label{tb:by_training_set_eu}
\end{table}

% tra1.0l10l22.00hyp0.31_tt_d32_20_64_mt0.12_dm4_hyper_lr0.005

% tra1.0 l10 l22.00 hyp0.3 1 _tt_d32_20_64_mt0.12_dm4_hyper_lr0.005


\begin{table}[t]
\small
\centering
\caption{Micro-averaged F1 for 12-class sentence-level aspect detection in restaurant reviews in Spanish with different ratios of training set r.}
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{1}{*}{}} 
& \multicolumn{5}{c|}{Restaurant review domain (Sp)}
\\
\multicolumn{1}{|l|}{\multirow{1}{*}{ratio r}} &
\multicolumn{1}{c}{10\%}&
\multicolumn{1}{c}{30\%}&
\multicolumn{1}{c}{50\%}&
\multicolumn{1}{c}{70\%}&
\multicolumn{1}{c|}{100\%}\\
\hline \multicolumn{1}{|l|}{{W2V-Gold}} & \multicolumn{1}{c}{{51.5}} &
\multicolumn{1}{c}{{62.4}} &
\multicolumn{1}{c}{{68.6}} &
\multicolumn{1}{c}{{71.3}} &
\multicolumn{1}{c|}{{74.6}}  \\
\multicolumn{1}{|l|}{{BERT-Gold}} & \multicolumn{1}{c}{{38.9}} &
\multicolumn{1}{c}{{47.6}} &
\multicolumn{1}{c}{{52.6}} &
\multicolumn{1}{c}{{59.3}} &
\multicolumn{1}{c|}{{65.0}}  \\
\hline 
\multicolumn{1}{|l|}{{MATE}} &
\multicolumn{1}{c}{{45.1}} &
\multicolumn{1}{c}{{54.8}} &
\multicolumn{1}{c}{{62.6}} &
\multicolumn{1}{c}{{67.4}} &
\multicolumn{1}{c|}{{72.8}}  \\
\multicolumn{1}{|l|}{{TS-ATT}} & \multicolumn{1}{c}{{49.5}} &
\multicolumn{1}{c}{{57.6}} &
\multicolumn{1}{c}{{67.0}} &
\multicolumn{1}{c}{{71.8}} &
\multicolumn{1}{c|}{{76.8}}   \\
\multicolumn{1}{|l|}{{TS-BT}} & \multicolumn{1}{c}{{40.3}} &
\multicolumn{1}{c}{{47.3}} &
\multicolumn{1}{c}{{53.5}} &
\multicolumn{1}{c}{{61.8}} &
\multicolumn{1}{c|}{{67.8}}  \\
\multicolumn{1}{|l|}{{\system}} &
\multicolumn{1}{c}{{\textbf{66.4}}} &
\multicolumn{1}{c}{{\textbf{68.7}}} &
\multicolumn{1}{c}{{\textbf{71.5}}} &
\multicolumn{1}{c}{{\textbf{74.5}}} &
\multicolumn{1}{c|}{{\textbf{78.7}}} \\
\hline 
\end{tabular}
\label{tb:by_training_set_sp}
\end{table}

% l10l25.00hyp0.11_tt_d32_10_64_mt0.12_dm4_hyper_lr0.005

% tra1.0l10l25.00hyp0.30.5_tt_d32_20_64_mt0.12_dm4_hyper_lr0.005


\begin{table}[t]
\small
\centering
\caption{Micro-averaged F1 for 12-class sentence-level aspect detection in restaurant reviews in French with different ratios of training set r.}
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{1}{*}{}} 
& \multicolumn{5}{c|}{Restaurant review domain (Fr)}
\\
\multicolumn{1}{|l|}{\multirow{1}{*}{ratio r}} &
\multicolumn{1}{c}{10\%}&
\multicolumn{1}{c}{30\%}&
\multicolumn{1}{c}{50\%}&
\multicolumn{1}{c}{70\%}&
\multicolumn{1}{c|}{100\%}\\
\hline \multicolumn{1}{|l|}{{W2V-Gold}} & \multicolumn{1}{c}{{33.7}} &
\multicolumn{1}{c}{{45.3}} &
\multicolumn{1}{c}{{51.6}} &
\multicolumn{1}{c}{{55.1}} &
\multicolumn{1}{c|}{{60.3}}  \\
\multicolumn{1}{|l|}{{BERT-Gold}} & \multicolumn{1}{c}{{19.9}} &
\multicolumn{1}{c}{{27.8}} &
\multicolumn{1}{c}{{31.2}} &
\multicolumn{1}{c}{{33.6}} &
\multicolumn{1}{c|}{{41.6}}  \\
\hline 
\multicolumn{1}{|l|}{{MATE}} &
\multicolumn{1}{c}{{38.1}} &
\multicolumn{1}{c}{{51.3}} &
\multicolumn{1}{c}{{53.3}} &
\multicolumn{1}{c}{{57.3}} &
\multicolumn{1}{c|}{{62.2}}  \\
\multicolumn{1}{|l|}{{TS-ATT}} & \multicolumn{1}{c}{{35.1}} &
\multicolumn{1}{c}{{40.8}} &
\multicolumn{1}{c}{{47.2}} &
\multicolumn{1}{c}{{49.9}} &
\multicolumn{1}{c|}{{53.6}}   \\
\multicolumn{1}{|l|}{{TS-BT}} & \multicolumn{1}{c}{{47.6}} &
\multicolumn{1}{c}{{49.7}} &
\multicolumn{1}{c}{{51.5}} &
\multicolumn{1}{c}{{53.1}} &
\multicolumn{1}{c|}{{58.7}}  \\
\multicolumn{1}{|l|}{{\system}} &
\multicolumn{1}{c}{{\textbf{49.9}}} &
\multicolumn{1}{c}{{\textbf{53.1}}} &
\multicolumn{1}{c}{{\textbf{56.2}}} &
\multicolumn{1}{c}{{\textbf{62.3}}} &
\multicolumn{1}{c|}{{\textbf{67.0}}} \\
\hline 
\end{tabular}
\label{tb:by_training_set_fr}
\end{table}

% tra1.0l10l20.50hyp0.40.5_tt_d32_64_20_mt0.12_dm4_hyper_lr0.005


\begin{table}[t]
\small
\centering
\caption{Micro-averaged F1 for 12-class sentence-level aspect detection in restaurant reviews in Russian with different ratios of training set r.}
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{1}{*}{}} 
& \multicolumn{5}{c|}{Restaurant review domain (Ru)}
\\
\multicolumn{1}{|l|}{\multirow{1}{*}{ratio r}} &
\multicolumn{1}{c}{10\%}&
\multicolumn{1}{c}{30\%}&
\multicolumn{1}{c}{50\%}&
\multicolumn{1}{c}{70\%}&
\multicolumn{1}{c|}{100\%}\\
\hline \multicolumn{1}{|l|}{{W2V-Gold}} & \multicolumn{1}{c}{{49.3}} &
\multicolumn{1}{c}{{52.4}} &
\multicolumn{1}{c}{{58.3}} &
\multicolumn{1}{c}{{62.2}} &
\multicolumn{1}{c|}{{69.3}}  \\
\multicolumn{1}{|l|}{{BERT-Gold}} & \multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c|}{{}}  \\
\hline 
\multicolumn{1}{|l|}{{MATE}} &
\multicolumn{1}{c}{{22.6}} &
\multicolumn{1}{c}{{41.3}} &
\multicolumn{1}{c}{{47.8}} &
\multicolumn{1}{c}{{57.3}} &
\multicolumn{1}{c|}{{61.2}}  \\
\multicolumn{1}{|l|}{{TS-ATT}} & \multicolumn{1}{c}{{58.8}} &
\multicolumn{1}{c}{{59.1}} &
\multicolumn{1}{c}{{59.8}} &
\multicolumn{1}{c}{{61.1}} &
\multicolumn{1}{c|}{{63.5}}   \\
\multicolumn{1}{|l|}{{TS-BT}} & \multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{}} &
\multicolumn{1}{c|}{{}}  \\
\multicolumn{1}{|l|}{{\system}} &
\multicolumn{1}{c}{{\textbf{55.2}}} &
\multicolumn{1}{c}{{\textbf{61.3}}} &
\multicolumn{1}{c}{{\textbf{67.8}}} &
\multicolumn{1}{c}{{\textbf{71.5}}} &
\multicolumn{1}{c|}{{\textbf{76.8}}} \\
\hline 
\end{tabular}
\label{tb:by_training_set_ru}
\end{table}

% tra1.0l10l20.50hyp0.201_tt_d32_64_168_mt0.12_dm4_hyper_lr0.005

\begin{table}[t]
\small
\centering
\caption{Micro-averaged F1 for 12-class sentence-level aspect detection in restaurant reviews in Dutch with different ratios of training set r.}
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{1}{*}{}} 
& \multicolumn{5}{c|}{Restaurant review domain (Du)}
\\
\multicolumn{1}{|l|}{\multirow{1}{*}{ratio r}} &
\multicolumn{1}{c}{10\%}&
\multicolumn{1}{c}{30\%}&
\multicolumn{1}{c}{50\%}&
\multicolumn{1}{c}{70\%}&
\multicolumn{1}{c|}{100\%}\\
\hline \multicolumn{1}{|l|}{{W2V-Gold}} & \multicolumn{1}{c}{{42.3}} &
\multicolumn{1}{c}{{52.1}} &
\multicolumn{1}{c}{{55.6}} &
\multicolumn{1}{c}{{60.1}} &
\multicolumn{1}{c|}{{67.4}}  \\
\multicolumn{1}{|l|}{{BERT-Gold}} & \multicolumn{1}{c}{{42.1}} &
\multicolumn{1}{c}{{50.1}} &
\multicolumn{1}{c}{{52.4}} &
\multicolumn{1}{c}{{56.9}} &
\multicolumn{1}{c|}{{59.0}}  \\
\hline 
\multicolumn{1}{|l|}{{MATE}} &
\multicolumn{1}{c}{{42.3}} &
\multicolumn{1}{c}{{52.6}} &
\multicolumn{1}{c}{{61.3}} &
\multicolumn{1}{c}{{63.9}} &
\multicolumn{1}{c|}{{68.7}}  \\
\multicolumn{1}{|l|}{{TS-ATT}} & \multicolumn{1}{c}{{43.6}} &
\multicolumn{1}{c}{{51.9}} &
\multicolumn{1}{c}{{62.8}} &
\multicolumn{1}{c}{{70.4}} &
\multicolumn{1}{c|}{{67.1}}   \\
\multicolumn{1}{|l|}{{TS-BT}} & \multicolumn{1}{c}{{40.5}} &
\multicolumn{1}{c}{{43.2}} &
\multicolumn{1}{c}{{47.9}} &
\multicolumn{1}{c}{{56.9}} &
\multicolumn{1}{c|}{{61.2}}  \\
\multicolumn{1}{|l|}{{\system}} &
\multicolumn{1}{c}{{\textbf{58.5}}} &
\multicolumn{1}{c}{{\textbf{62.5}}} &
\multicolumn{1}{c}{{\textbf{68.3}}} &
\multicolumn{1}{c}{{\textbf{72.1}}} &
\multicolumn{1}{c|}{{\textbf{73.8}}} \\
\hline 
\end{tabular}
\label{tb:by_training_set_du}
\end{table}

% tra1.0l10l20.50hyp0.201_tt_d32_64_168_mt0.12_dm4_hyper_lr0.005


\begin{table}[t]
\small
\centering
\caption{Micro-averaged F1 for 12-class sentence-level aspect detection in restaurant reviews in Turkish with different ratios of training set r.}
\begin{tabular}{cccccccc}
\hline
\multicolumn{1}{|c|}{\multirow{1}{*}{}} 
& \multicolumn{5}{c|}{Restaurant review domain (Tur)}
\\
\multicolumn{1}{|l|}{\multirow{1}{*}{ratio r}} &
\multicolumn{1}{c}{10\%}&
\multicolumn{1}{c}{30\%}&
\multicolumn{1}{c}{50\%}&
\multicolumn{1}{c}{70\%}&
\multicolumn{1}{c|}{100\%}\\
\hline \multicolumn{1}{|l|}{{W2V-Gold}} & \multicolumn{1}{c}{{31.6}} &
\multicolumn{1}{c}{{41.2}} &
\multicolumn{1}{c}{{44.3}} &
\multicolumn{1}{c}{{50.8}} &
\multicolumn{1}{c|}{{55.7}}  \\
\multicolumn{1}{|l|}{{BERT-Gold}} & \multicolumn{1}{c}{{}} &
\multicolumn{1}{c}{{43.1}} &
\multicolumn{1}{c}{{48.6}} &
\multicolumn{1}{c}{{52.3}} &
\multicolumn{1}{c|}{{56.5}}  \\
\hline 
\multicolumn{1}{|l|}{{MATE}} &
\multicolumn{1}{c}{{40.2}} &
\multicolumn{1}{c}{{43.7}} &
\multicolumn{1}{c}{{46.1}} &
\multicolumn{1}{c}{{48.6}} &
\multicolumn{1}{c|}{{51.6}}  \\
\multicolumn{1}{|l|}{{TS-ATT}} & \multicolumn{1}{c}{{44.3}} &
\multicolumn{1}{c}{{45.9}} &
\multicolumn{1}{c}{{50.8}} &
\multicolumn{1}{c}{{52.4}} &
\multicolumn{1}{c|}{{53.5}}   \\
\multicolumn{1}{|l|}{{TS-BT}} & \multicolumn{1}{c}{{37.5}} &
\multicolumn{1}{c}{{41.9}} &
\multicolumn{1}{c}{{45.7}} &
\multicolumn{1}{c}{{50.1}} &
\multicolumn{1}{c|}{{55.6}}  \\
\multicolumn{1}{|l|}{{\system}} &
\multicolumn{1}{c}{{\textbf{51.6}}} &
\multicolumn{1}{c}{{\textbf{54.3}}} &
\multicolumn{1}{c}{{\textbf{58.9}}} &
\multicolumn{1}{c}{{\textbf{62.1}}} &
\multicolumn{1}{c|}{{\textbf{67.7}}} \\
\hline 
\end{tabular}
\label{tb:by_training_set_tur}
\end{table}

% l10l20.50hyp0.11_tt_d32_168_64_mt0.12_dm4_hyper_lr0.005

% tra1.0l10l20.10hyp0.41_tt_d32_64_20_mt0.12_dm4_hyper_lr0.005

==> case_st_boots_2.tex <==

\begin{table*}[t]
\fontsize{9}{10}\selectfont
\center
\small
\scalebox{1.0}{
\noindent\begin{tabular}{|c|c|c|c|c|}
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{But may be unsightly.}} &
\multicolumn{1}{c|}{GT: Look} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: cute, look, looked, great, fringe, great, fringe, style, color, love, design, going, unattractive, attractive}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Durability $\color{red}\XSolidBrush$} &
% bag
\multicolumn{1}{|c|}{{MATE: Size $\color{red}\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{However, I bought them in February.}} &
\multicolumn{1}{c|}{GT: General} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: return, pair, thought, year, boot, high, kind, merrell, excited, wore, disappointed, buy, problem}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: General $\color{blue} \Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Price $\color{red}\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{blue} \Checkmark$}} 
\\
\hlin
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{I ordered these a half-size up}} &
\multicolumn{1}{c|}{GT: Size} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: size, ordered, half, order, big, little, bigger, usually, narrow, normally, width}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Size $\color{blue} \Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: General $\color{red}\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: Size $\color{blue} \Checkmark$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{Nice looking shoes.}} &
\multicolumn{1}{c|}{GT: Look} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: cute, look, looked, great, fringe, great, fringe, style, color, love, design, going, unattractive, attractive}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Look $\color{blue} \Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Look $\color{blue} \Checkmark$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: Color $\color{red}\XSolidBrush$}} 
\\
\hlin
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{Hurt after 30 minutes}} &
\multicolumn{1}{c|}{GT: Comfort} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: comfortable, fit, foot, hurt, ankle, comfy, blister, comfort, break, wear, able, extreme, walking, sock}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Comfort $\color{blue}$  $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Comfort $\color{blue}$  $\Checkmark$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: Comfort $\color{blue}$  $\Checkmark$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{The material is very thin and flimsy}} &
\multicolumn{1}{c|}{GT: Materials} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: leather, inside, fringe, material, heel, cheaper, soft, sole, buckle, suede, true, rubber, advertised}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Materials $\color{blue} \Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Materials $\color{blue} \Checkmark$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: Materials $\color{blue} \Checkmark$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{Which helps in the Maine {$\color{red}$winter}.}} &
\multicolumn{1}{c|}{GT: Weather resistance} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: dry, waterproof, rain, wet, water, foot, soaked, {$\color{red}$snow}, {$\color{red}$cold}, puddle, warm, got, chicago, protect, suppose}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Weather resistance $\color{blue}$ $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: General $\color{red}$ $\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}$ $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{It was a washed {$\color{red}$purplish} but not a true {$\color{red}$purple}}} &
\multicolumn{1}{c|}{GT: Color} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: {$\color{red}$color}, love, {$\color{red}$style}, unbelievably, gorgeous, blue, favorite, taupe, wonderful, red, exactly, design}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Color $\color{blue}$ $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Size $\color{red}$ $\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}$ $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{I wanted a true {$\color{red}$purple} boot.}} &
\multicolumn{1}{c|}{GT: Color} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: {$\color{red}$color}, love, style, unbelievably, gorgeous, blue, favorite, taupe, wonderful, red, exactly, design}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Color $\color{blue}$  $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: General $\color{red}$ $\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: Price $\color{red}$  $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{That I can easily {$\color{red}$slip on} and not {$\color{red}$struggle} to put it on.}} &
\multicolumn{1}{c|}{GT: Comfort} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: comfortable, {$\color{red}$fit}, foot, hurt, ankle, comfy, blister, {$\color{red}$comfort}, break, {$\color{red}$wear}, able, extreme, walking, sock}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Comfort $\color{blue}$   $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Comfort $\color{blue}$  $\Checkmark$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}$  $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{They seem pretty {$\color{red}$solid} to me.}} &
\multicolumn{1}{c|}{GT: Durability} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: rubber, quality, use, buckle, appear, heel, {$\color{red}$long}, time, {$\color{red}$breaking}, enjoy, provide}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Durability $\color{blue}$  $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Durability $\color{blue}$   $\Checkmark$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}$  $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{And {$\color{red}$scratch up} your fingers getting your foot into the things though.}} &
\multicolumn{1}{c|}{GT: Comfort} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: {$\color{red}$comfortable}, fit, foot, hurt, ankle, comfy, blister, comfort, break, wear, able, extreme, walking, sock}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Comfort $\color{blue}$   $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: General $\color{red}$  $\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: Weather Resistance $\color{red}$ $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{It would {$\color{red}$stay tied} as well.}} &
\multicolumn{1}{c|}{GT: Durability} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: rubber, quality, use, buckle, appear, heel, {$\color{red}$long}, time, breaking, enjoy, provide, {$\color{red}$protection}, clearly, cheaply}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Durability $\color{blue}$  $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Look $\color{red}$ $\XSolidBrush$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}$ $\XSolidBrush$}} 
\\
\hline 
\multicolumn{2}{|l}{\multirow{1}{*}{You need to design these with a {$\color{red}$zipper}.}} &
\multicolumn{1}{c|}{GT: Materials} 
\\
% \hline
\multicolumn{3}{|l|}{\multirow{1}{*}{Seed Words: leather, inside, fringe, {$\color{red}$material}, heel, cheaper, soft, sole, buckle, suede, true, rubber, advertised}}
\\
\hline
\multicolumn{1}{|c|}{$\system$: Materials $\color{blue}$  $\Checkmark$} &
% bag
\multicolumn{1}{|c|}{{MATE: Materials $\color{blue}$  $\Checkmark$}} &
% B/T 
\multicolumn{1}{c|}{{TS-W2V: General $\color{red}$ $\XSolidBrush$}} 
\\
\hline 
\end{tabular}}
\caption{Comparison of predictions on sample Boots product review segments between $\system$, MATE, and TS-W2V. For each review segment, the ground true (GT) aspect and its corresponding seed words are provided.}
\vspace{-1.5 pc}
\label{tb:case_st_kb}
\end{table*}

